ReAl: Refine neural operators via aligning dynamical flow

Neural partial differential equation (PDE) surrogates trained with mean squared error (MSE) can capture dominant dynamics but often lose high-frequency information and fine-scale structures. Generative models (e.g., Flow Matching) can capture the distribution of fine-scale details, yet stochastic errors may accumulate during autoregressive rollouts and compromise long-term stability. To address these limitations, we introduce Refine and Align(ReAl), a model-agnostic plug-in that augments pretrained PDE surrogates to improve the reconstruction of high-frequency structures associated with complex physical phenomena. In the refinement stage, a conditional flow-matching model learns the residual distribution around the deterministic base prediction, recovering missing fine-scale structures while retaining the dominant dynamics. In the alignment stage, to mitigate the generative discrepancies amplified in the autoregressive rollout, particularly in chaotic systems, we generate multiple trajectories from the same input and reinforce the refiner with trajectory-level rewards, thereby achieving long-horizon dynamical alignment. Experiments across diverse surrogate architectures and PDE tasks demonstrate that ReAl consistently improves high-frequency fidelity, forecasting accuracy, and long-horizon stability.

==> chapter/introduction.tex <==

\section{Introduction}

% PDE领域目前的发展，神经算子的发展

% Partial differential equations (PDEs) provide a fundamental mathematical framework for describing the evolution of physical systems in the natural sciences and engineering, with applications spanning fluid mechanics~\citep{davidson2004turbulence05}, heat and mass transfer~\citep{bergman2011fundamentals}, electromagnetics~\citep{schwinger1998classical07}, and chemical diffusion~\citep{crank1979mathematics08}. Although classical numerical discretization techniques, including finite-difference schemes~\citep{morton1994numerical01} and finite-element methods~\citep{hughes2003finite02}, can produce reliable  solutions, their computational burden increases rapidly with spatial resolution, problem dimensionality, and the size of parameter studies. This limitation has motivated growing interest in deep-learning-based PDE surrogates and operator-learning approaches, such as DeepONet~\citep{lu2021learning03}, the Fourier Neural Operator~\citep{li2020fourier04}, and the Physics-Informed Neural Operator~\citep{goswami2023physics09}. By approximating the underlying solution operators, these methods can substantially reduce inference costs and offer an effective computational pathway for large-scale simulations and real-time scientific prediction.

Partial differential equations (PDEs) are fundamental to modeling physical systems across fluid mechanics~\citep{davidson2004turbulence05}, heat and mass transfer~\citep{bergman2011fundamentals}, electromagnetics~\citep{schwinger1998classical07}, and chemical diffusion~\citep{crank1979mathematics08}. Classical finite-difference~\citep{morton1994numerical01} and finite-element methods~\citep{hughes2003finite02} provide reliable solutions, but their computational costs grow rapidly with spatial resolution, dimensionality, and parameter-space size. This limitation has driven the development of deep-learning-based PDE surrogates and neural operators, including DeepONet~\citep{lu2021learning03}, the Fourier Neural Operator~\citep{li2020fourier04}, and the Physics-Informed Neural Operator~\citep{goswami2023physics09}. By approximating PDE solution operators, these methods enable substantially faster inference for large-scale simulation and real-time scientific prediction.


Most deep-learning-based PDE surrogates are trained with mean squared error (MSE) objective, which provides stable optimization and effectively captures large-scale, low-frequency dynamics. 
However, as a mean-regression objective, MSE tends to suppress
high-frequency information, local vortices, and sharp interfaces
~\citep{lippe2023pde11,fotiadis2024stochastic12}, particularly on real-world datasets such as RealPDEBench~\citep{hu2026realpdebench}, where measurement noise and unresolved physical processes further
complicate the underlying dynamics.
Generative models~\citep{ho2020denoising19, rombach2022high20, lipman2022flow21} can alleviate this limitation by modeling the
conditional distribution of PDE solutions instead of producing only
one deterministic prediction, enabling richer high-frequency details~\citep{yao2026guided14,utkarsh2026physics,hu2025wavelet16}. However, stochastic sampling may introduce predictive variance and compromise the dynamical consistency and long-term stability required by deterministic PDE systems. 


Motivated by these observations, we adopt a complementary modeling strategy: retain the MSE-trained surrogate as a stable predictor of dominant dynamics and apply a conditional flow-based refiner to its output. Rather than regenerating the entire PDE state, the refiner is
conditioned on the base prediction and learns to generate its
fine-scale residual correction~\citep{fotiadis2024stochastic12}. As shown in Fig.\ref{fig:intro}~\subref{fig:intro1}, this strategy recovers high-frequency information lost by MSE training while preserving low-frequency dynamics consistent in PDE predictions. Despite these benefits, a generative refiner can only partially
mitigate the rollout shift rather than completely eliminate it. Stochastic perturbations can accumulate during autoregressive rollout, and the refiner’s generation objective is not fully aligned with the base surrogate’s forecasting objective, creating a mismatch between local detail correction and general dynamics~\citep{luo2025pdespectralrefiner, Yoo2026DiffusionRolloutUR13}. As shown in Fig.\ref{fig:intro}~\subref{fig:intro2}, the base model preserves low-frequency dynamics over longer horizons, while high-frequency errors progressively accumulate and amplify, degrading long-term stability and physical consistency.





To further mitigate this limitation, inspired by reinforcement learning for diffusion models~\citep{Liu2025FlowGRPOTF17,zheng2026diffusionnft18},
we introduce trajectory-alignment post-training for the flow-based
refiner. Starting from the same input state, we sample multiple
autoregressive trajectories using independent random seeds and evaluate their long-term quality with trajectory-level rewards. These rewards reinforce residual corrections that produce accurate, stable, and physically consistent trajectories while suppressing those that cause error accumulation. This extends the optimization target from
one-step accuracy to long-term trajectory quality without sacrificing
the refiner's ability to recover fine-scale structures. Our main
contributions are summarized as follows:




\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.435\textwidth}
        \centering
        \includegraphics[width=\linewidth]{image/intro1.pdf}
        \caption{Necessity of refinement}
        \label{fig:intro1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.535\textwidth}
        \centering
        \includegraphics[width=\linewidth]{image/intro2.pdf}
        \caption{Necessity of alignment}
        \label{fig:intro2}
    \end{subfigure}
    \caption{(a) MSE training leads to high-frequency information loss, while stochastic refiner recovers the structures. (b) Sampling variability accumulates during stochastic autoregressive rollout, especially in the high-frequency regime. Our ReAl mitigates this accumulation of sampling variability.}
    \label{fig:intro}
\end{figure*}

\roxie{remember to update this one.}
% \textbf{Our contirbutions:}
% In summary, we propose a unified PDE forecasting framework that
% integrates deterministic base prediction, stochastic 
% refinement, and trajectory-level policy optimization.
% % Our main contributions are summarized as follows: \textcolor{red}{modify}

\begin{itemize}
\item We propose \textbf{Re}fine and \textbf{Al}ign \textbf{(ReAl)}, a lightweight, model-agnostic PDE forecasting plug-in based on Flow Matching. ReAl addresses the loss of high-frequency information and fine-scale structures commonly observed in MSE-pretrained surrogates on real-world data, refining their predictions without modifying the underlying architectures.

\item To the best of our knowledge, we are the first to post-train long-term autoregressive PDE trajectories from a reinforcement learning perspective. \textbf{ReAl} samples multiple stochastic rollouts from the same initial state and optimizes the Flow refiner with trajectory-level rewards, aligning local residual corrections with long-term dynamical evolution.

\item Extensive experiments demonstrate that \textbf{ReAl} improves both prediction accuracy and long-term stability. Compared with the base models, it reduces the average RMSE by $34.3\%$ at the first rollout step and by $45.4\%$ at the $20$-th step, with larger gains over longer horizons on RealPDEBench. \textbf{ReAl} also recovers high-frequency physical structures, suppresses long-term error accumulation, and mitigates numerical dissipation.
\end{itemize}

% Given an MSE-pretrained PDE surrogate, it
% combines stable modeling of dominant dynamics, fine-scale residual
% recovery through a conditional Flow refiner, and long-horizon alignment
% through trajectory-level FlowNFT post-training. 

==> chapter/method.tex <==
\section{Method}
\label{sec:method}

% In this section, we present our framework for stable and accurate
% long-term Partial differential equation(PDE) forecasting, as illustrated in
% Fig.~\ref{fig:trajectory_nft1}. Our framework uses an MSE-pretrained PDE
% surrogate as a deterministic backbone and augments its predictions with
% a conditional Flow-based generative refiner. The surrogate captures the
% dominant dynamics, while the refiner generates fine-scale residual
% corrections that are missing from the base prediction. To align local refinement with long-term PDE evolution, we introduce
% trajectory-level FlowNFT post-training to optimize the refiner using
% rewards from multi-step autoregressive rollouts, explicitly targeting
% long-term accuracy, stability, and physical consistency. 

In this section, we introduce \textbf{Re}fine and \textbf{Al}ign (\textbf{ReAl}), a model-agnostic plug-in for stable and accurate long-term partial differential equation forecasting, as illustrated in Fig.~\ref{fig:trajectory_nft1}. During refinement, we pretrain a flow matching refiner to correct the residual distribution of the base predictions. During alignment, we employ trajectory-level post-training to improve long-term forecasting stability.



\subsection{Preliminaries}
\noindent\textbf{PDE surrogates for forecasting.}
% MSE-trained rollout simulator， rollout 长程
Consider a nonlinear dynamical system governed by a partial differential equation (PDE):
\begin{equation}
\frac{\partial \boldsymbol{u}}{\partial t}
=
\mathcal{G}(\boldsymbol{u};\phi),
\label{eq1:pde_dynamics}
\end{equation}
% \roxie{boldsymbol or mathbf?}
where \(\boldsymbol{u}(\boldsymbol{x},t)\) denotes a continuous physical field depending on spatial coordinate \(\boldsymbol{x}\) and time $t$, \(\phi\) represents the physical parameters governing the dynamics of the system, and $
\mathcal{G}: \mathcal{U} \times \Phi \rightarrow\mathcal{U}$ is a differential operator. By applying numerical discretization techniques, such as finite-difference or spectral methods, we obtain a discrete trajectory of consecutive observed states:$\{\boldsymbol{u}_0,\boldsymbol{u}_1,\ldots,\boldsymbol{u}_N\}$. Our goal is to learn a neural surrogate
model $f_\theta$, parameterized by $\theta$, that approximates the discrete
evolution operator and predicts the next state
$\boldsymbol{u}_{n+1}$ from the current state
$\boldsymbol{u}_n $\footnote{To simplify the notation, we consider one-step forecasting as a
representative setting. Our method is agnostic to the temporal
input--output configuration and can be applied to surrogates that use
multiple historical states or predict multiple future states.},
$\hat{\boldsymbol{u}}_{n+1}=f_\theta(\boldsymbol{u}_n).$
 For multi-step forecasting, the surrogate model is applied recursively in an autoregressive manner. The prediction at the \(k\)-th future step is given by $\hat{\boldsymbol{u}}_{n+k}
= f_{\theta}^{\circ k}(\boldsymbol{u}_n),$ where $f_{\theta}^{ \circ k}(\cdot)$ denotes the $k$-fold composition of
$f_{\theta}(\cdot)$.

% While the MSE-trained surrogate provides a stable deterministic
% prediction, its regression objective lacks the ability to model the
% conditional distribution of unresolved fine-scale structures. We therefore introduce conditional
% flow matching, which forms the generative foundation of our stochastic
% refiner.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth,
        trim=0.5cm 0cm 0cm 0cm,
        clip]{image/method1.pdf}
    \caption{Overview of \textbf{Re}fine and \textbf{Al}ign (\textbf{ReAl}), a model-agnostic plug-in
for pretrained PDE surrogates. (a) \textbf{Refine}: a conditional flow matching 
refiner generates fine-scale residuals for the frozen deterministic
prediction. (b) \textbf{Align}: trajectory rewards from multiple
stochastic rollouts post-train the refiner for stable long-term PDE
forecasting.}
    \label{fig:trajectory_nft1}
\end{figure*}

\noindent\textbf{Conditional Flow Matching.} 
Conditional flow matching (CFM)~\citep{lipman2022flow21} learns a conditional vector field that
transports samples from a Gaussian noise distribution to the target
data distribution conditioned on $\boldsymbol{c}$. During training, an
intermediate state is sampled along a linear interpolation between a
noise sample and a target sample, and the vector field
$\boldsymbol{v}_{\psi}$ is optimized to predict the corresponding
transport velocity. At inference, the learned vector field is integrated
from noise to data to generate a sample under the given condition.
Here, the flow time $\tau\in[0,1]$ parameterizes the generative transport
process and is distinct from the physical time of PDE evolution.
% Conditional flow matching (CFM) learns a conditional vector field that
% transports noise
% $\boldsymbol{z}_0\sim\mathcal{N}(\boldsymbol{0},\boldsymbol{I})$
% to a target sample
% $\boldsymbol{z}_1\sim p_{\mathrm{data}}(\cdot\mid\boldsymbol{c})$.
% Using the linear path
% \begin{equation}
%     \boldsymbol{z}_{\tau}
%     =
%     (1-\tau)\boldsymbol{z}_0
%     +
%     \tau\boldsymbol{z}_1,
%     \qquad
%     \tau\sim\mathcal{U}(0,1),
%     \label{eq:cfm_path}
% \end{equation}
% the vector field $\boldsymbol{v}_\psi$ is trained by:
% \begin{equation}
%     \mathcal{L}_{\mathrm{CFM}}(\psi)
%     =
%     \mathbb{E}
%     \left[
%     \left\|
%     \boldsymbol{v}_\psi
%     (\boldsymbol{z}_\tau,\tau\mid\boldsymbol{c})
%     -
%     (\boldsymbol{z}_1-\boldsymbol{z}_0)
%     \right\|_2^2
%     \right].
%     \label{eq:cfm_objective}
% \end{equation}

% At inference, the learned vector field is integrated from $\tau=0$ to
% $\tau=1$ to generate a sample conditioned on $\boldsymbol{c}$. Here,
% $\tau$ denotes the generative flow time and should be distinguished
% from the temporal evolution state of the PDE rollout.


% \subsection{Flow matching refiner}

\subsection{Distribution Refinement with Conditional Flow Matching}
\label{sec:stochastic_refinement}

We first introduce the distribution refinement phase of \textbf{ReAl}, as shown in Fig.~\ref{fig:trajectory_nft1}(a). Most existing PDE surrogates are trained with MSE, enabling the deterministic predictor $\boldsymbol{d}_{\theta}$ to stably capture dominant dynamics but often suppressing high-frequency structures through mean regression. To address this limitation, we introduce a conditional flow matching refiner $\boldsymbol{g}_{\psi}$ that learns the residual distribution between the base prediction and ground truth, recovering fine-scale structures.




% Given the current PDE state $\boldsymbol{u}_n$, our goal is to construct a
% transition operator $\boldsymbol{f}_{\theta,\phi}$ that predicts the subsequent
% state $\boldsymbol{u}_{n+1}$. As illustrated in Fig.~2(a), the transition
% consists of two sequential components: an MSE-pretrained deterministic predictor
% $\boldsymbol{d}_{\theta}$ and a stochastic Flow-based residual refiner
% $\boldsymbol{g}_{\phi}$. The former captures stable dominant dynamics, while
% the latter models residual corrections for unresolved fine-scale structures.


\noindent\textbf{Deterministic Base Prediction.}
Given the current PDE state $\boldsymbol{u}_n$, the MSE-based
deterministic predictor produces the next-state estimate, $\bar{\boldsymbol{u}}_n$, and is
pretrained by minimizing its discrepancy from the ground truth, $\boldsymbol{u}_{n+1}$:

\begin{equation}
\begin{aligned}
\bar{\boldsymbol{u}}_{n+1}=
\boldsymbol{d}_{\theta}(\boldsymbol{u}_n),~~~~
\mathcal{L}_{\mathrm{MSE}}(\theta)
=
\mathbb{E}
\left[
\left\|
\bar{\boldsymbol{u}}_{n+1}
-
\boldsymbol{u}_{n+1}
\right\|^2
\right].
\end{aligned}
\label{eq:deterministic_predictor}
\end{equation}

% Let $\boldsymbol{c}_n$ denote the forecasting condition, with
% $\boldsymbol{c}_n=\boldsymbol{u}_n$ in the one-step setting. The deterministic
% branch produces
% \begin{equation}
%     \tilde{\boldsymbol{u}}_{n+1}
%     =
%     \boldsymbol{d}_{\theta}(\boldsymbol{c}_n),
% \end{equation}
% and is pretrained using
% \begin{equation}
%     \mathcal{L}_{\mathrm{MSE}}
%     =
%     \mathbb{E}
%     \left[
%         \left\|
%         \boldsymbol{d}_{\theta}(\boldsymbol{c}_n)
%         -
%         \boldsymbol{u}_{n+1}
%         \right\|_2^2
%     \right].
% \end{equation}
The optimal MSE predictor approaches the conditional mean,
   $
    \mathbb{E}
    \left[
        \boldsymbol{u}_{n+1}\mid\boldsymbol{u}_n
    \right].$ Although this reliably captures the dominant dynamics, conditional averaging tends to suppress non-dominant fine-scale structures, resulting in overly smooth predictions.


\noindent\textbf{Conditional Flow Refinement.}
To recover non-dominant structures suppressed by MSE training, we introduce a conditional flow matching refiner \(\boldsymbol{g}_{\psi}\) that models the conditional distribution of fine-scale residuals. Specifically, we define the target residual, $\boldsymbol{r}_{n+1}$, and the condition, $\boldsymbol{c}_n$, as:
\begin{equation}
\begin{aligned}
\boldsymbol{r}_{n+1}
=
\boldsymbol{u}_{n+1}
-
\bar{\boldsymbol{u}}_{n+1},~~~~
\boldsymbol{c}_n
=
\operatorname{Concat}
\left[
\boldsymbol{u}_n,
\bar{\boldsymbol{u}}_{n+1}
\right].
\end{aligned}
\end{equation}

The refiner learns to generate \(\boldsymbol{r}_{n+1}\) conditioned on the current state, $\boldsymbol{u}_{n}$, and deterministic base prediction, $\bar{\boldsymbol{u}}_{n+1}$.
Given a Gaussian sample \(\boldsymbol{z}_0\sim\mathcal{N}(\boldsymbol{0},\boldsymbol{I})\), we construct a linear flow path toward the target residual:
\begin{equation}
\boldsymbol{z}_{\tau}
=
(1-\tau)\boldsymbol{z}_0
+
\tau\boldsymbol{r}_{n+1},
\qquad
\tau\sim\mathcal{U}(0,1).
\label{eq:method_z}
\end{equation}

The conditional velocity field \(\boldsymbol{v}_{\psi}\) is trained to match the corresponding transport velocity:
\begin{equation}
\mathcal{L}_{\mathrm{refine}}(\psi)
=
\mathbb{E}
\left[
\left\|
\boldsymbol{v}_{\psi}
\left(
\boldsymbol{z}_{\tau},
\tau
\mid
\boldsymbol{c}_n
\right)
-
\left(
\boldsymbol{r}_{n+1}
-
\boldsymbol{z}_0
\right)
\right\|^2
\right].
\end{equation}

At inference, the generative mapping \(\boldsymbol{g}_{\psi}\) is obtained by integrating \(\boldsymbol{v}_{\psi}\) from \(\tau=0\) to \(\tau=1\), starting from \(\boldsymbol{\epsilon}\sim\mathcal{N}(\boldsymbol{0},\boldsymbol{I})\). The generated residual and refined prediction are:
\begin{equation}
\begin{aligned}
\hat{\boldsymbol{r}}_{n+1}
=
\boldsymbol{g}_{\psi}
\left(
\boldsymbol{\epsilon}
\mid
\boldsymbol{c}_n
\right),~~~~
\hat{\boldsymbol{u}}_{n+1}
=
\bar{\boldsymbol{u}}_{n+1}
+
\hat{\boldsymbol{r}}_{n+1}.
\end{aligned}
\end{equation}
 The deterministic predictor and stochastic refiner are complementary: the former captures stable dominant dynamics, while the latter restores residual fine-scale structures without imposing a strict low- and high-frequency decomposition, as illustrated in Fig.~\ref{fig:trajectory_nft1}(a).
% \subsection{Deterministic Prediction with Stochastic Flow Refinement}


% Given the current PDE state \(\boldsymbol{u}_n\), our goal is to learn a transition operator \(f_{\theta,\psi}\) that maps \(\boldsymbol{u}_n\) to the subsequent state \(\boldsymbol{u}_{n+1}\). We construct \(f_{\theta,\psi}\) using two sequentially connected components: $f_{\theta,\psi}=d_\theta \circ g_\psi$, where \(d_\theta\) is an MSE-based deterministic predictor that captures the dominant dynamics, and \(g_\psi\) is a stochastic Flow-based refiner that supplements the deterministic prediction with fine-scale residual information, as shown in~Fig.\ref{fig:trajectory_nft1}(a).

% % \(d(\cdot)\) — deterministic，确定性动力学分支
% % \(g(\cdot)\) — generative，生成动力学分支




% The deterministic and generative branches have different prediction
% objectives. Given the forecasting condition $c_n$, the deterministic
% branch directly predicts the next physical state by minimizing
% \begin{equation}
% \mathcal{L}_{\mathrm{MSE}}
% =
% \mathbb{E}
% \left[
% \left\|
% \boldsymbol d_{\theta}(c_n)
% -
% \boldsymbol u_{n+1}
% \right\|_2^2
% \right].
% \end{equation}
% Its optimal solution is the conditional mean
% \begin{equation}
% \boldsymbol d^*(c_n)
% =
% \mathbb{E}
% [\boldsymbol u_{n+1}\mid c_n].
% \end{equation}
% Therefore, MSE regression is effective for capturing predictable and
% dominant dynamics. However, when multiple future states are compatible
% with the same condition, averaging their positions, amplitudes, or
% phases can suppress structures that are not consistently aligned.

% MSE also weights errors according to their absolute magnitude. In the
% Fourier domain, Parseval's identity gives
% \begin{equation}
% \left\|
% \hat{\boldsymbol u}-\boldsymbol u
% \right\|_2^2
% =
% \sum_{\boldsymbol k}
% \left|
% \hat{\boldsymbol U}_{\boldsymbol k}
% -
% \boldsymbol U_{\boldsymbol k}
% \right|^2 .
% \end{equation}
% Consequently, high-amplitude dominant modes contribute more to the
% total loss than low-amplitude, non-dominant modes. Under limited model
% capacity and optimization, such weak modes may be insufficiently
% constrained. These modes are often associated with high-frequency
% structures, although low amplitude and high frequency are not
% equivalent.

% Flow Matching instead learns a conditional transport process. Given a
% source state $\boldsymbol z_0$ and target state
% $\boldsymbol z_1=\boldsymbol u_{n+1}$, it defines
% \begin{equation}
% \boldsymbol z_r
% =
% (1-r)\boldsymbol z_0+r\boldsymbol z_1,
% \qquad r\in[0,1],
% \end{equation}
% and trains a velocity field using
% \begin{equation}
% \mathcal{L}_{\mathrm{FM}}
% =
% \mathbb{E}
% \left[
% \left\|
% \boldsymbol v_{\phi}(\boldsymbol z_r,r;c_n)
% -
% (\boldsymbol z_1-\boldsymbol z_0)
% \right\|_2^2
% \right].
% \end{equation}
% Although this objective also uses a squared error, it regresses the
% local transport velocity rather than the final physical state. By
% sampling different source states, Flow Matching can represent
% different plausible future trajectories instead of collapsing them into
% a single conditional mean.

% Motivated by these complementary properties, we construct a sequential
% two-stage architecture:
% \begin{equation}
% \tilde{\boldsymbol u}_{n+1}
% =
% \boldsymbol d_{\theta}(c_n),
% \qquad
% \hat{\boldsymbol u}_{n+1}
% =
% \boldsymbol g_{\phi}
% \left(
% \tilde{\boldsymbol u}_{n+1},
% \boldsymbol\epsilon;c_n
% \right),
% \quad
% \boldsymbol\epsilon\sim\mathcal N(\boldsymbol 0,\boldsymbol I).
% \end{equation}
% The deterministic branch provides a coherent prediction of the
% dominant dynamics, while the subsequent Flow Matching branch refines
% the prediction by modeling residual errors and conditional variability.
% The two branches are therefore complementary rather than strict
% low-frequency and high-frequency filters.




\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{image/method_mean_var.pdf}
    \caption{Qualitative results on Controlled Cylinder \textit{Real2Real} for velocity components \(u\) and \(v\). Residuals are computed against the ground truth, while variance is measured across random seeds. Base+ReAl produces more accurate and consistent predictions.
    }
    \label{fig:method_mean_var}
\end{figure*}



\subsection{Trajectory Alignment for PDE Forecasting}

Although combining the deterministic predictor
$\boldsymbol{d}_{\theta}$ with a conditional flow matching refiner
$\boldsymbol{g}_{\psi}$ recovers non-dominant fine-scale information
missing from the base prediction, perturbations introduced by stochastic
flow sampling may accumulate during autoregressive rollouts and degrade
long-term stability. To address this issue, we introduce the
trajectory-alignment post-training phase of \textbf{ReAl}, as shown in Fig.~\ref{fig:trajectory_nft1}(b). Specifically,
we keep $\boldsymbol{d}_{\theta}$ frozen and post-train the refiner
$\boldsymbol{g}_{\psi}$ using trajectory-level rewards from multiple
stochastic rollouts, thereby improving the quality of long-term PDE
trajectories.



\noindent\textbf{Trajectory rollout.}
Given an initial state \(\boldsymbol{u}_n\), we generate \(K\) candidate trajectories using the frozen deterministic predictor \(\boldsymbol{d}_{\theta}\) and a snapshot of the refiner \(\boldsymbol{g}_{\psi}^{\mathrm{old}}\). All candidates start from the same state but use independent noise sequences. For the \(i\)-th candidate, we initialize \(\hat{\boldsymbol{u}}^{(i)}_n=\boldsymbol{u}_n\) and recursively apply the refined transition:
\begin{equation}
\begin{aligned}
\bar{\boldsymbol{u}}^{(i)}_{n+k}
&=
\boldsymbol{d}_{\theta}
\left(
\hat{\boldsymbol{u}}^{(i)}_{n+k-1}
\right),
\boldsymbol{c}^{(i)}_{n+k-1}
=
\operatorname{Concat}
\left[
\hat{\boldsymbol{u}}^{(i)}_{n+k-1},
\bar{\boldsymbol{u}}^{(i)}_{n+k}
\right], \\
\hat{\boldsymbol{r}}^{(i)}_{n+k}
&=
\boldsymbol{g}_{\psi^{\mathrm{old}}}
\left(
\boldsymbol{\epsilon}^{(i)}_k
\mid
\boldsymbol{c}^{(i)}_{n+k-1}
\right),
\quad
\boldsymbol{\epsilon}^{(i)}_k
\sim
\mathcal{N}(\boldsymbol{0},\boldsymbol{I}), \\
\hat{\boldsymbol{u}}^{(i)}_{n+k}
&=
\bar{\boldsymbol{u}}^{(i)}_{n+k}
+
\hat{\boldsymbol{r}}^{(i)}_{n+k},
\quad
k=1,\ldots,h.
\end{aligned}
\end{equation}

After \(h\) autoregressive steps, the resulting trajectory is:
\begin{equation}
\widehat{\mathcal{T}}^{(i)}_n
=
\left[
\hat{\boldsymbol{u}}^{(i)}_{n+1},
\hat{\boldsymbol{u}}^{(i)}_{n+2},
\ldots,
\hat{\boldsymbol{u}}^{(i)}_{n+h}
\right],
\qquad
i=1,\ldots,K.
\end{equation}
Despite sharing the same initial state and deterministic predictor, independent residual samples produce different long-term trajectories. As shown in Fig.~\ref{fig:method_mean_var}, stochastic refinement (\(\text{Base}+\text{Re}\)) introduces high-frequency variance that can accumulate during autoregressive rollouts.


\noindent\textbf{Trajectory-level reward.}
Each candidate trajectory $\widehat{\mathcal{T}}^{(i)}_n$ is evaluated against the corresponding ground-truth trajectory $\mathcal{T}_n$ to obtain its trajectory-level reward:

\begin{equation}
\begin{aligned}
R^{(i)}
=
\mathcal{R}
\left(
\widehat{\mathcal{T}}^{(i)}_n,
\mathcal{T}_n
\right), \quad
R^{(i)}_{\mathrm{MSE}}
=
-
\left\|
\hat{\boldsymbol{u}}^{(i)}_{n+h}
-
\boldsymbol{u}_{n+h}
\right\|^2,
\end{aligned}
\label{eq:trajectory_reward}
\end{equation}
where \(R^{(i)}_{\mathrm{MSE}}\) denotes the negative mean squared error at the terminal state, such that a larger reward indicates a more accurate terminal prediction. Although the reward is evaluated only at the endpoint, the terminal state reflects the accumulated effects of stochastic residual corrections propagated throughout the multi-step autoregressive rollout. It therefore serves as a measure of long-term trajectory quality. More generally, \(\mathcal{R}\) may be defined using discrepancies in physically relevant quantities, such as vorticity, divergence, and kinetic energy, or by combining multiple criteria to evaluate complementary properties of the predicted dynamics.

Since reward magnitudes can vary across initial conditions, we
standardize the rewards within each group of $K$ trajectories. Let $\mu_R$ and $\sigma_R$ denote the group
mean and standard deviation, respectively. We then clip the standardized
reward and linearly rescale it to $[0,1]$:
\begin{equation}
w^{(i)}
=
\frac{1}{2}
\left[
1+
\frac{1}{a_{\max}}
\operatorname{clip}
\left(
\frac{R^{(i)}-\mu_R}
{\sigma_R+\epsilon_{\mathrm{num}}},
-a_{\max},
a_{\max}
\right)
\right].
\label{eq:reward_weight}
\end{equation}
Here, $\epsilon_{\mathrm{num}}$ is a small constant that ensures
numerical stability and \(a_{\max}>0\) controls the clipping range. Consequently, higher-quality trajectories receive
weights closer to $1$, whereas lower-quality receive
weights closer to $0$. 


\noindent\textbf{Trajectory reward-Guided Flow Alignment.}
Our objective is to increase the likelihood of generating high-quality
long-horizon trajectories while reducing the likelihood of low-quality
ones. For the $k$-th autoregressive transition of the $i$-th candidate
trajectory, $\boldsymbol{z}^{(i,k)}_{\tau}$ denotes the intermediate
residual state at flow time $\tau$, following
Eq.~\eqref{eq:method_z}. The velocity fields predicted by the
current policy, old policy, and reference model are uniformly written as:
\begin{equation}
\boldsymbol{v}^{s,(i,k)}
=
\boldsymbol{v}_{\psi^{s}}
\left(
\boldsymbol{z}^{(i,k)}_{\tau},
\tau
\mid
\boldsymbol{c}^{(i)}_{n+k-1}
\right),
\qquad
s\in
\left\{
\mathrm{cur},
\mathrm{old},
\mathrm{ref}
\right\}.
\label{eq:trajectory_velocity_fields}
\end{equation}
Here, $\psi^{\mathrm{cur}}\equiv\psi$ denotes the parameters of the
refiner being updated, $\psi^{\mathrm{old}}$ denotes the old-policy
parameters used to generate the candidate trajectories, and
$\psi^{\mathrm{ref}}$ denotes the parameters of the pretrained reference
model, which remain frozen throughout post-training. Following the negative-aware forward-process formulation of
DiffusionNFT~\citep{zheng2026diffusionnft18}, we construct positive and
negative velocity fields from the current- and old-policy predictions:
\begin{equation}
\begin{aligned}
\boldsymbol{v}^{+,(i,k)}
=
\beta\boldsymbol{v}^{\mathrm{cur},(i,k)}
+
(1-\beta)\boldsymbol{v}^{\mathrm{old},(i,k)}, \quad
\boldsymbol{v}^{-,(i,k)}
=
(1+\beta)\boldsymbol{v}^{\mathrm{old},(i,k)}
-
\beta\boldsymbol{v}^{\mathrm{cur},(i,k)},
\end{aligned}
\label{eq:positive_negative_velocity}
\end{equation}
where $\beta>0$ controls the deviation of the positive and negative
velocity fields from the old policy. The corresponding positive and negative flow matching losses are:
\begin{equation}
\ell_{\pm}^{(i,k)}
=
\left\|
\boldsymbol{v}^{\pm,(i,k)}
-
\left(
\boldsymbol{r}^{(i)}_{n+k}
-
\boldsymbol{z}^{(i,k)}_0
\right)
\right\|^2.
\label{eq:local_positive_negative_loss}
\end{equation}

The final alignment objective averages over both candidate trajectories
$i$ and autoregressive steps $k$:
\begin{equation}
\mathcal{L}_{\mathrm{align}}
=
\frac{1}{\beta}
\mathbb{E}_{i,k}
\left[
w^{(i)}\ell_{+}^{(i,k)}
+
\left(1-w^{(i)}\right)\ell_{-}^{(i,k)}
\right].
\label{eq:flow_alignment}
\end{equation}
Same trajectory-level reward \(w^{(i)}\) is applied to every autoregressive step of the \(i\)-th candidate. A high trajectory reward produces a weight close to \(1\), emphasizing the positive objective and encouraging the associated residual corrections. A low reward produces a weight closer to \(0\), emphasizing the negative objective. Because the same trajectory-level weight is shared at every rollout step, the terminal feedback supervises residual generation along the entire trajectory.

To stabilize post-training, we further regularize the refiner
toward the frozen pretrained reference model while retaining the
supervised residual-learning objective. The training objective is:
\begin{equation}
\mathcal{L}
=
\mathcal{L}_{\mathrm{align}}
+
\lambda_{\mathrm{ref}}
\mathbb{E}_{i,k}
\left[
\left\|
\boldsymbol{v}^{\mathrm{cur},(i,k)}
-
\boldsymbol{v}^{\mathrm{ref},(i,k)}
\right\|^2
\right]
+
\lambda_{\mathrm{sup}}
\mathbb{E}_{i,k}
\left[
\left\|
\hat{\boldsymbol{r}}^{(i)}_{n+k}
-
\boldsymbol{r}^{(i)}_{n+k}
\right\|^2
\right].
\label{eq:post_training_objective}
\end{equation}
The reference-model regularization prevents excessive deviation from the
pretrained flow dynamics, while the supervised term preserves the
refiner's residual-modeling capability. Throughout post-training, only
the current refiner parameters $\psi$ are updated; the deterministic
predictor $\boldsymbol{d}_{\theta}$, old-policy parameters
$\boldsymbol{g}_{\psi}^{\mathrm{old}}$, and reference-model parameters
$\boldsymbol{g}_{\psi}^{\mathrm{ref}}$ remain frozen.

Overall, \textbf{ReAl} produces more accurate long-term predictions with lower across-seed variance. By favoring residual corrections that remain reliable over long horizons, it produces more accurate predictions with lower across-seed variance, as shown in Fig.~\ref{fig:method_mean_var} (Base+ReAl).

